Configurable calorimeter simulation for AI applications

A configurable calorimeter simulation for AI (COCOA) applications is presented, based on the Geant4 toolkit and interfaced with the Pythia event generator. This open-source project is aimed to support the development of machine learning algorithms in high energy physics that rely on realistic particle shower descriptions, such as reconstruction, fast simulation, and low-level analysis. Specifications such as the granularity and material of its nearly hermetic geometry are user-configurable. The tool is supplemented with simple event processing including topological clustering, jet algorithms, and a nearest-neighbors graph construction. Formatting is also provided to visualise events using the Phoenix event display software.

==> sections_old/dataProcessing.tex <==

%%Although the SCD is built inheriting the geometry of the ATLAS detector, the difference is nevertheless sufficient to have various parameterization for native ATLAS topological clustering and particle flow (\textbf{PFlow}) algorithms ~\cite{Aad_2017, Aaboud_2017}  of post-processing algorithms used in ATLAS for SCD implementation.

\pat{
    Among the event reconstruction algorithms provided by SCD, the jet clustering
    makes use of FastJet~\cite{Cacciari_2012} as an external library with configurable choices for the clustering algorithm and parameters. The Topo-Clustering and particle flow algorithms on the other hand are implemented within SCD and work similarly to the corresponding algorithms used by the ATLAS collaboration.
}
%
%
% The FASTJET authors want us to also cite hep-ph/0512210 . But we don't have to,
% or ? PR.
%
%

\subsection{Topological clustering}

\textbf{TODO: Sanmay, check if the topo-clustering remark discussed with Marumi on 05(09/22 is in here.}

%The finite resolution of the calorimeter system still makes it possible
%to trace the spatial developing energy shower from incoming particles.
%The topological clustering algorithm performs two crucial tasks: separation particle showers of different nature (i.e., electromagnetic and hadronic) from each other by forming topological clusters (topo-clusters) and noise-suppression.
%The algorithm starts the cluster maker procedure by forming proto-clusters using seeding calorimeter cells whose signal value divided by the  nominal noise level exceeds a certain threshold $S$ ($S=4$ in ATLAS).
%The proto-clusters then grow by iteratively adding all neighboring cells with absolute signal $N$ ($N=2$ in ATLAS) times above nominal noise.
%Once no more neighboring cells can be found above the $N$ threshold, the cluster maker procedure is finished by %adding all cells adjacent to the cells already in proto-clusters.

\pat{
While SCD provides deposited energies per calorimeter cell for downstream tasks which look deeply into
detector signatures, for convenience a clustering of these cells is provided as well.
This topological clustering algorithm serves the separation of electromagnetic and hadronic
showers and the suppression of noise. The seeding cluster cells are required to contain a deposited
energy well above the noise level, where the threshold of this signal-to-noise ratio (SNR)
amounts to 4.5 for the ATLAS experiment and 4.0 for SCD by default. The difference is chosen in order to achieve
a better agreement between ATLAS and SCD in terms of the cluster multiplicity distribution for single
charged and neutral pions as well as pure noise events (Fig.~\ref{fig:Topo}).
Starting with the seeding cells, all neighbouring cells are added to the cluster if their SNR is below another threshold, where a default value amounts to 2. Finally, all further neighbouring cells are added independently
of their amount of deposited energy.
}
\textbf{ToDo: This paragraph doesn't sound correct. To be discussed. PR.} If proto-cluster has more than one local energy maxima, i.e., cells with energy above $500$ GeV, it is split between those maxima to consider the spatial distribution of energy within a single proto-cluster and improve the reconstruction objects accuracy.
%
%For the SCD, only $S$ is different from ATLAS implementation and is set to be equal to 4.5 to achieve similar distribution for the number of reconstructed clusters for simulated charged and neutral single pions and empty events.
%
%Formed topo-clusters are treated as distinct four-momentum objects in event reconstruction.
\pat{
The energies of the resulting topo-clusters are added and the resulting vector is provided in the SCD output file.
}


%\begin{figure}[ht]
%    \centering
%    {\includegraphics[width=1\linewidth]{fig/From_t%hesis/Plots/TopoClust.pdf}}
%\caption{The number of reconstructed clusters for %single-particle events with charged and neutral %pions and empty events in SCD using the default %topo-clustering parameters.}
%\label{fig:Topo}
%\end{figure}

\begin{figure*}
    \centering
    \subcaptionbox{ $\sigma_\eta$ distribution}[0.45\textwidth]{\includegraphics[width=1.1\linewidth]{fig/nTC.pdf}}
    \hfill
    \subcaptionbox{$\sigma_\phi$ distribution. }[0.45\textwidth]{\includegraphics[width=1.1\linewidth]{fig/averageE.pdf}}
  
\caption{The number of reconstructed clusters for
single-particle events with charged and neutral
pions and empty events in SCD using the default
topo-clustering parameters.}
\label{fig:Topo}
\end{figure*}


\subsection{Particle flow}
%The PFlow algorithm aims to resolve overlap between energy deposited by electrically neutral and charged particle showers of charged hadrons and other particles (exclude muons and neutrinos) in calorimeters. Resolving the overlapping problem is made it possible to use the combination of momentum and energy measurements from the tracker and calorimeter system. As a result, particle flow reconstruction can significantly improve event reconstruction precision.

\pat{
PFlow reconstruction algorithms combine the charged particle tracks measured
by inner tracking detectors with the energy deposits of calorimeters in order
to assign these deposits to either charged or neutral particles. The energy of
the charged particles is associated with the momentum measurement of the tracking
detector rather than calorimeter energy deposits, due to the higher accuracy of
the track momentum compared to calorimeter energy measurements
of hadrons. This technique has been established both in the ATLAS and CMS collaborations
and an implementation similar to the one used by ATLAS is provided by SCD.
It serves as a benchmark to which new, more sophisticated reconstruction algorithms
can be compared.
}




\begin{figure*}
    \centering
    \subcaptionbox{ $\sigma_\eta$ distribution}[0.45\textwidth]{\includegraphics[width=1\linewidth]{fig/From_thesis/Plots/Fig10eta_new.pdf}}
    \hfill
    \subcaptionbox{$\sigma_\phi$ distribution. }[0.45\textwidth]{\includegraphics[width=1.\linewidth]{fig/From_thesis/Plots/Fig10phi_new.pdf}}
  
\caption{\textbf{ToDo: more information here. Refer to it in the text. PR.}The distribution of $\sigma_\eta$  and $\sigma_\phi$ for charged pions with three different $p_T^\text{true}$ bins in $|\eta^{\text{true}}|<1.0$ region.}
\label{fig:sigmaeta}
\end{figure*}

% Parametrization of charge hadrons energy subtraction procedure strongly depends on detector features and topo-clusters formation.
%Therefore, the implementation of the SCD particle flow algorithm requires a complete calibration process. 
%The algorithm starts from selecting tracks that that are not associated with electrons or muons, able to reach the first calorimeter layer, and within $\left|\eta\right|<3.0$.
%For each selected track, PFlow makes an attempt to match a single topo-cluster in the calorimeter system. 
\pat{
The SCD PFlow algorithm first selects tracks which are not associated with
electrons or muons and able to reach the first calorimeter layer.
\textbf{ToDo: what does that mean ("reach"), some pT threshold? PR.}
For each of these tracks a corresponding topo-cluster is seeked.
\textbf{ToDo: how is the matching defined? Also, the rest of the paragraph
we should discuss to make it more precise. PR.}
}
Then, based on track $p_T$, $\eta$, and layer with the largest rate of increase in energy density for a given track, the expected energy deposition is computed.
Since single-particle deposition can be split among several topo-clusters, the algorithm estimates whether associate track with more than one topo-clusters and with which one of them.


%Cell by cell subtraction from the set of matched topo-clusters starts from forming a list of rings around the track, ordered according to their energy density and with a radius equal to a single cell pitch in each calorimeter layer. 
%Energy from the calorimeter system is then subtracted starting from the ring with the highest energy density. 
%The subtraction proceeds until the total amount of removed energy exceeds the expected energy. 
%If the ring's energy is larger than the energy that remains to be subtracted, then the energy in cells in this ring is scaled to the fraction needed to reach the expected energy.
%Finally, if the remaining energy in the matched topo-clusters, after subtraction of all rings energy, are less than expected shower fluctuations for a given track, all remnants are removed.


\pat{
For topo-clusters matched to a track, the expected deposited energies are subtracted.
For this purpose, rings are formed around the track and ordered according to their
energy density. The ring width amounts to a single cell pitch in each calorimeter layer.
The ring energies are subtracted consecutively until the total subtracted matches
the expected energy.
\textbf{ToDo: Where does the expectation come from? PR.}
Finally, if the remaining energy of the topo-cluster is below the amount of energy
fluctuation corresponding to the matched track, all of its remaining energy is removed as well.
}

\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{fig/DeltaRprime_2_5GeV.pdf}
    \caption{\textbf{ToDo: More info. Reference in the text. PR.} Track to cluster association optimization.}
    \label{fig:DeltaRprime_2_5GeV}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{fig/S_epsilon_5_10GeV.pdf}
    \caption{\textbf{ToDo: More info. Reference in the text. PR.} Optimization of energy fluctuation of topocluster.}
    \label{fig:S_epsilon_5_10GeV}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% I suggest to put the tracking module before the PFlow stuff. PR.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Tracking Module}
\textbf{ToDo: This section should be rewritten completely.
I can hardly follow it, so have a hard time with rewriting it.
Also, why do we need all these formulas in the paper? PR.}
The tracking procedure in the absence of measurements from the inner detector is made by calculating perigee parameters of track with radius $\rho = p_T/0.3B_z$ in magnetic field $B_z$ from the initial coordinates $(x^{init},y^{init},z^{init})$ and initial momenta $(p_x^{init},p_y^{init},p_z^{init})$ of final state particles with charge $q$

\begin{equation}
    \left\{ \begin{aligned} 
        a_0&=\left(\sqrt{x_0^2+y_0^2}-\rho\right)q\\
        z_0&=z_{init}-2\rho \cot{\theta}\arcsin{\sqrt{\frac{x^2_{init}+y^2_{init}-a_0^2}{4\rho^2+4q a_0 \rho}}}\\
        \varphi_0 &= \arctan{y_0/x_0}+\frac{1}{2}q\pi\\
        \cot & \theta=\frac{p_z}{p_T}\\
        q_{p_T}&=\frac{q}{p_T}
    \end{aligned}\right.,
\end{equation}
where $x_0=x_{init}+q\rho \frac{p_y}{p_T}$ and $y_0=y_{init}-q\rho \frac{p_x}{p_T}$ coordinate of the centre  of helix in $x-y$ plane.
Each calculated perigee parameter is smeared using Gaussian distribution with width dependent on track $p_T$ to introduce a finite resolution of track parameters measured by the inner detector. 
\textbf{ToDo: We should describe the track smearing more quantitatively and point out why we use the values we use. PR.}

Tracks extrapolation to the beginning of calorimeter system in barrel or end-cap region is made using smeared perigee parameters
\begin{equation}
    \left\{ \begin{aligned} 
        x&=(q a_0 +\rho)\cos\left(\phi_0-q\frac{\pi}{2}\right)+
        q\rho \sin\left(q\varphi-\varphi_0\right)\\
        y&=(q a_0 +\rho)\sin\left(\phi_0-q\frac{\pi}{2}\right)+
        q\rho \cos\left(q\varphi-\varphi_0\right)\\
        z&=z_0+\rho \phi \cot{\theta}\\
    \end{aligned}\right.,
\end{equation}
\textbf{ToDo: Not clear to me what is going on here. PR.}
where $\varphi$ is a parameter.   
All tracks are saved, including those who do not take part in further event reconstruction: tracks produced outside second silicon pixel layer, tracks that do not reach the calorimeter system, tracks , and tracks marked as unreconstructed, to model track reconstruction efficiency.
\textbf{ToDo: Doesn't make sense, right? We don't look at where a track is produced because we don't have real tracks. PR.}

\section{Truth Matching}
\textbf{ToDo: This section should really come right after "Detector Design". A dedicated single section for this might not be needed. PR.}

%Stable particles are generated by event generators like Pythia or particle gun and these particle traverse through the tracking volume before entering the calorimeter of the designed detector. 
%During these passage, the charged particles are bent by the magnetic field and neutral particles fly by without changing the direction and eventually all of them enter the calorimeter volume. 

%\pat{
Primary, stable particles are introduced at the IP using the PYTHIA event generator~\cite{pythia} or simply a single particle gun.  As these particles traverse the detector, their interaction
with the detector material is simulated by GEANT in a sequence of short steps. For interactions in the calorimeter, SCD records the  deposited energy of the affected calorimeter cell and assigns it to the primary particle which caused the interaction.
Electron-positron pairs from photon conversions taking place
in the ITS upstream its two outermost iron layers are identified
and stored in the SCD output file.
%}

%Apart from neutrinos and muons, rest of the particles starts releasing their energies through 
%electromagnetic and hadronic interactions. The energy deposition for a given particle happens through a series of short steps. Inside the GEANT4  package, these steps are executed through a class called "SteppingAction". A series of steps make up the whole trajectory created by the energy deposition from a particle. A single trajectory is accessed through a class named "TrackingAction" within the simulation framework.

\textbf{ToDo: What's the point of the following paragraph? PR.}
In the current working environment, for a given event, typically we have hundreds of shower trajectories, each consisting of few thousands of steps and often these steps are overlapping with each other in the same geometrical region of the detector. Hence it becomes a highly challenging combinatorial task to correctly assign a given shower step to trajectory and eventually associate a trajectory to an unique truth particle.
In SCD we keep track of each shower evolution history to assign a truth particle origin to each shower step.


==> sections_old/detectorDesign.tex <==
%The  Simplified Cylindrical Detector (SCD) is designed to inherit the common broad features of a %general-purpose LHC detector but omitting the engineering sophistication of a state of the art %real detector.  SCD is  built up of inner tracking system(ITS), electromagnetic calorimeter %(ECAL) and hadronic calorimeter (HCAL). 
%Each subdetector component is cylindrical in shape and stacked to each other in the radial %direction with ITS being the innermost and HCAL being the outermost volume, respectively. The %sub-detector volumes are split in several layers, both along radial and transverse direction, as %shown in Fig.~\ref{fig:Barrel_EndCap_scheme}.

The SCD contains all major components needed to emulate the reponse of a general-purpose LHC detector. It is simplified by the exclusion of engineering components like cabling, readout sensors and grounded support structures. A muon spectrometer
is not required due to the presence of the ITS. The subdetectors are cylindrical and stacked on top of each other in the order ITS, ECAL, HCAL. While the ITS consists of
cylinders and discs, the calorimeters are segmented in both the radial and longitudinal direction, as shown in Fig.~\ref{fig:Barrel_EndCap_scheme}.



%A major requirement of this software design is to make the detector parameters customizable through user input. 
%Layers' granularity and width, together with other parameters of the calorimeter system described below, are easy to set up through the JSON configuration file.
%What follows is a description of the default detector configuration, which is meant to emulate the ATLAS detector.

\pat{In case of the default configuration, SCD is similar to the ATLAS detector.}
%The closest part of the detector to the interaction point is the inner tracking system (\textbf{ITS}).
%A uniform axial 3.8 Tesla magnetic field is applied to the ITS region.
%From the collision point outward, the ITS consist of five 150 $\mu m$ silicon layers to mimic the silicon pixel detector and four 320 $\mu m$ silicon layers to mimic the semiconductor tracker.
%Each of those layers has an additional outer 350 $\mu m$ layer of iron to imitate support material. 
%ITS layers are represented by hollow cylinders nested inside each other around the beam axis and followed, in the $z$ direction, by disks perpendicular to the beam axis as shown in Fig.~\ref{fig:Barrel_EndCap_scheme}.
%The ITS does not perform the function of measuring momentum but instead adds material in the path of incoming particles and provokes a shower in front of the calorimeter system, bringing the SCD closer to reality.

The ITS consists of hollow cylinders in the central detector part and disks at both of its ends, each of which are centered around the beamline. Each of these components consists of a silicon layer of 150~\mum thickness in case of the disks and the five innermost cylinders and 320~\mum in case of the 4 outermost cylinders.
%
%
% IS THAT REALLY WHAT WE WANT?? PR.
%
%
Each silicon layer is accompanied by an iron layer of 350 \mum thickness in order to simulate support material.
The ITS only serves the purpose of simulating the interaction of particles with matter. The resulting detector hits
are not used for tracking purposes. The smearing approach to charged particle tracking used in SCD is described further
below.
The default value of the magnetic flux density present in the ITS amounts to 3.8~T.

Finally, two layers of iron were added to represent the transition radiation tracker and other material in front of the calorimeter system.



%The calorimeter system, the next sub-detector that appears on the way of incoming particles shown in Fig~\ref{fig:Barrel_EndCap_scheme}, composed of two parts: electromagnetic (\textbf{ECAL}) and hadronic (\textbf{HCAL}) calorimeters that have uniform segmentation in $\eta$ and $\phi$ directions designed to energy measurement with high spatial resolution.
%Each part consist of three layers, with different width and varying granularity, presented as cylinders in barrel region ($|\eta|<1.5$) and as discs in end-caps regions ($1.5<|\eta|<3.0$), sequentially situated one after another.

\pat{
The calorimeter system is stacked on top of the iron layers closing the cylindrical ITS and separated into a barrel ($|\eta|<1.5$) and end-cap ($1.5<|\eta|<3.0$) region.
Both the ECAL and the HCAL are divided into 3 layers stacked on top of each other. The cell granularity can be configured for each calorimeter layer individually.
The calorimeter cells are designed such that in every layer each of them covers the same distance in terms of pseudorapidity and azimuthal angle, such that an approximately uniform distribution of incoming particles is obtained from hadron collisions at the interaction point (IP). Furthermore, the depth of the cells of every layer is constant in order to ensure that the layer fractions of deposited energy do not depend on the incoming particle direction. This design, leading to layer shapes of the form $1\,/\,\cosh{\eta}$, is similar to the ATLAS and CMS ECAL design and makes SCD better suited for shower learning tasks than a simple rectangular calorimeter design.}


%The real detector components in ATLAS detector are sampling calorimeter with absorber and scintillator as sub-components. The ECAL of CMS is a homogeneous calorimeter. In our simulation, we apply equivalent molecule approximation to design the detector material as a mixture of absorber and scintillator material
%with pre-determined proportion. This makes the homogeneous material to act as an absorber and the scintillator at the same time. %The ECAL is modeled as a homogeneous calorimeter by mixing lead and liquid argon, corresponds to ATLAS calorimeter materials, in volume proportion $1:3.83$, achieving radiation length of $X_0 = 2.5$ cm. 
%For the HCAL, iron, as the absorber material, and polyvinyl toluene plastic material, as a scintillating active material, are mixed with a volume proportion $1.1.:1.0$ yielding to nuclear interaction length $\lambda_{int}=26.6$ cm.

\pat{
The SCD calorimeter material is a compound using an equivalent molecule approximation, mixing an absorber and scintillator material with a constant proportion. Both the materials and their proportion can be configured for the ECAL
and the HCAL individually. By default, the ECAL is made of a mixture of lead and liquid argon, corresponding to the ATLAS ECAL materials. The volume proportion amounts to $1:3.83$, resulting in a radiation length of $X_0 = 2.5$ cm.
The ECAL and HCAL are separated by an iron layer with a default thickness of 80\,mm.
The HCAL is made of a mixture of iron and polyvinyl toluene plastic material with a volume proportion of  $1.1.:1.0$, resulting in a nuclear interaction length of $\lambda_{int}=26.6$ cm.
}
The integrated radiation and interaction length measured from the IP to the end of the HCAL is shown as a function
of the pseudorapidity in Fig~\ref{fig:Rad_Int_length}.

%The simulated energy deposits in each layer are then smeared as $\sigma_E/E=1/\sqrt{E}$ to reproduce the corresponding sampling energy resolution.
%The electronic noise from measuring devices and pile-up effect from several events that happen simultaneously and are counted as a single event are mimicked using normal distributions centered at zero with variables widths for different layers.
%The choice of material and smearing parameters are tuned to reproduce single-particle response of ATLAS calorimeter system.
%In Table~\ref{tab:CaloLaeyrs}, one can find default values for granularity, width, and noise level in calorimeter cells for each calorimeter layer.

\pat{
In order to take sampling fluctuations into account, the simulated energy deposits in each cell, $E$, are smeared using a centered Gaussian distribution with a standard deviation of $\sqrt{E}$.
Noise from electronic readout and additional primary ineractions is simulated by the addition of random amounts of energy
following a centered Gaussian distribution with configurable standard deviations for each calorimeter layer.
The default choices of materials and smearing parameters, provided in Tab.~\ref{tab:CaloLaeyrs} are tuned in order to approximate single-particle responses of the ATLAS calorimeter system.
}


%\subsection{High-resolution detector}

%It was shown by Di Bello et al.~\cite{Di_Bello_2021} that a super-resolution approach in deep learning can improve spatial energy distribution reconstruction.
%For the purpose of developing such techniques, the SCD supports simulating a higher granularity version along with a low-resolution (standard resolution) of the detector calorimeter response on an event. Neural Network then trained to predict the high-resolution version from the standard one. The output from the trained network then is used as an input that can have many applications, one of them the electron and photon identification that allows separating strong overlap showers making particle flow algorithms more accurate.

%Similarly, as it was for the standard resolution version, the SCD allows setting up a high-resolution version of the detector in both longitudinal and transverse directions by increasing amount of cells in each layer and slicing each layer into several smaller, respectively.
%Low-resolution cells response is not the result of the separately generated event but the consequence of the summation constituent high-resolution cells.




%
% Rad. length and int. length: is that slang? Do we need to add "elm." and "had.", resp.? PR.
%

\begin{table}[]
    \centering
    \caption{\color{red}{TODO: CHECK VALUES BEFORE RELEASE.}
    %Widths, in corespondent radiation $X_0$ \TODO{update?} and interaction $\lambda_{int}$ lengths, granularity, and the Gaussian distribution widths (the nominal noise) of simulated noise for each calorimeter layer are shown.
    \pat{
    Calorimeter default design regarding layer depths in terms of radiation length $X_0$ (ECAL) and interaction length $\lambda_{int}$ (HCAL), granularity and noise.
    }
    }
    \begin{tabular}{l|ccc}
            & Width                               &  Granularity ($\eta \times \phi$)                      & Noise {[}MeV{]} \\ \hline
        ECAL1 & $4X_0$                            & $256 \times 256$ & 13               \\
        ECAL2 & $16X_0$                           & $256 \times 256$ & 34               \\
        ECAL3 & $2X_0$                            & $128 \times 128$ & 41               \\ \hline
        HCAL1 & $1.5\lambda_{int}$                & $64 \times 64$ & 75               \\
        HCAL2 & $4.1\lambda_{int}$                & $64 \times 64$ & 50               \\
        HCAL3 & $1.8\lambda_{int}$                & $32 \times 32$ & 25               \\
    \end{tabular}
    \label{tab:CaloLaeyrs}
\end{table}



\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{fig/scd_yz_xy.pdf}
    \caption{Positive quadrant scheme of the SCD. (left) yz-projection demonstrates ITS and calorimeter system in the barrel and end-caps regions. (right) xy-projection shows barrel region of ITS and calorimeter system. }
    \label{fig:Barrel_EndCap_scheme}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{fig/geantinoScan_scdDefaultDesign_150922.pdf}
    \caption{(left) Cumulative amounts of material, in units of radiation length $X_0$ and as a function
of $\eta$, in front of and in the electromagnetic calorimeter system. (right) Cumulative amounts of material, in units of interaction length $\lambda_{int}$ and as a function
of $\eta$, in front of and in the hadronic calorimeter system.}
    \label{fig:Rad_Int_length}
\end{figure*}
% \begin{figure*}
%     \centering
%     \includegraphics[width=1\textwidth]{fig/Jet_Particle_Responce_IronGap.pdf}
%     \caption{}
%     % \label{fig:Barrel_EndCap_scheme}
% \end{figure*}






% \begin{figure*}
%     \centering
%     \includegraphics[width=0.8\textwidth]{fig/SCDdesign.pdf}
%     \caption{General structure of the SCD code}
%     \label{fig:scd_design}
% \end{figure*}


==> sections_old/eventDisplay.tex <==

\textbf{ToDo: Decide if we want to have an event display here. Also decide if we mention the event displays shipped with SCD at all (not that there are 3 of them). PR.}
Access to the information on the truth level allows one to have a closer look at what is happening during the event. This ability leads to creating an HTML-based interactive event display that gives access to results of full event simulation and separate processes during the event.

The figure shows the complete graph of the hadronization process for 14 TeV pp collision and its detector response, and the figure shows the sub-process of W decay and detector measurements of its product that's happened during this event. 

\textbf{ToDo: Conclusion? PR.}


==> sections_old/introduction.tex <==

%Statistical analysis on simulated monte-carlo (MC)
%events are crucial part of any high energy physics
%research program.
%The simulated samples are used as
%template for well understood physics processes
%which can be reliably used for new physics study.
%The templates are also used to validate newly built
%frameworks.



%A dedicated high energy event simulation using the full detector simulation is a computation heavy task and often solely done through dedicated effort within large experimental collaboration and such simulated samples are seldom available to the world outside these collaborations. The computational codes, used to produce these MC samples, are often released in open platforms. However, producing reliable bulk simulated samples using these are often beyond the scope of individual practitioner.

\fdb{do we really want to introduce the framework like this? I would just say that this is a flexible package for quick ML developments. Without mentioning large experiments. The statements made are also debatable such as “Huge computing efforts and expertise regarding the complex underlying computer codes” this is only because we don’t make public our datasets in a smart manner… not a limitation per se. }
Experimental data in High Energy Physics (HEP) is \newline
recorded by complex detectors and its interpretation depends on Monte-Carlo (MC)
simulations of these detectors. Large experimental collaborations operating such detectors control detailed simulations
accordingly. In parallel, research efforts dedicated to the reconstruction of collision events in HEP are also pursued outside of these collaborations. The independent research groups cannot make use of the simulation infrastructure used within the collaborations as they require huge computing efforts and expertise regarding the complex underlying computer codes. Furthermore the resulting simulated event samples are usually not publicly available.
In order to streamline the independent development of reconstruction technqiues in HEP and in order to allow for fair comparisons of the resulting algorithms, a common detector simulation is desired.


%In the recent times we have software frameworks
%like Delphes \cite{Mertens:2015kba}, which
%implements parametric smearing on final state
%object kinematics to emulate realistic detector
%smearing effects. These kind of frameworks are very
%useful for phenomenological studies. However, the
%energy shower caused inside detector material due
%to passage of energetic particle is solely missing 
%from such packages. For accessing realistic shower 
%profile, we need to run GEANT simulation toolkit \cite{ALLISON2016186}.


Depending on the required level of accuracy, different approaches to such independent simulations can be chosen.
A fast and popular approach is to apply parametric smearing functions to primary particle momenta in order to emulate detector responses,
as implemented in the Delphes framework~\cite{Mertens:2015kba}. This approach is suited to studies of particle physics phenomenology,
for instance to test if a new physics model is expected to result in sizeable detector signals.
On the other hand, the development of new experimental techniques requires to go way beyond this smearing approach,
taking into account the details of the interactions between particles and detector material as provided by
the GEANT simulation toolkit\\~\cite{ALLISON2016186}.

%Lately, learning of shower profiles using deep neural networks have gain popularity and several attempts have been made as can be found in the %articles \cite{PhysRevD.97.014021,Qasim_2019,Di_Bello_2021}. All of these studies attempt to learn realistic shower pattern, sticking to simplified %detector configuration. While the simplified detector implementation is readily available from GEANT templates, a full cylindrical detector having all %the general features of a general purpose experiment at LHC is not readily available. 
Prime examples of such developments are recent and ongoing research efforts to distinguish shower profiles caused by different particles
in dense material, using deep neural networks~\cite{PhysRevD.97.014021,Qasim_2019,Di_Bello_2021}. These studies make use of simple detector
geometries like rectangular blocks divided into cells of equivalent size. In order to train and test the algorithms under study in a more realistic
setting, a detector design including major features of the general purpose experiments at the LHC is desired, but it has not been available so far.


%In this project we design a fully hermitic cylindrical detector with multiple layers of electromagnetic calorimeter (ECAL) and hadronic calorimeter (HCAL) using GEANT, such that the 
%single particle responses of the proposed calorimeter matches  closely with the typical LHC values and one can perform reliable physics studies using such a framework.

%
% What do we have here? A letter? A paper? Something else? PR.
%

This letter presents the Simplified Cylindrical Detector (SCD), which implements the desired detector design based on GEANT. The major components of the SCD are its electromagnetic (ECAL) and hadronic calorimeter (HCAL), designed to suit the needs of hadron collision analysis. Single particle responses of the SCD calorimeters closely match those of the multipurpose LHC detectors. The main parameters of the calorimeters are largely configurable through a JSON file, including their material, granularity, depth and the amount of readout noise. SCD also includes an inner tracking system (ITS) made of silicon tracking and supporting iron layers, the incorporation of which is subject to the choice of the user. The space surrounded by the calorimeters is filled by a magnetic field of adjustable strength. Several reconstruction algorithms are provided with SCD for user convenience, namely topological clustering of calorimeter cell energies,
particle flow reconstruction and jet clustering.

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.7\textwidth]{fig/SCD.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure*}

==> sections_old/introduction_old.tex <==
\mk{the introduction is a tricky exercise for this paper. The general idea is that it should stay as simple and factual as possible i.e. not much more than what is in the abstract, but it should explain why this is for AI application. One aspect that could be emphasised is that this can be used more broadly than in the HEP community and this is why it is important to use ML friendly notations. It should explain why it is a 'simplified' simulation, this is because it has a very simplified 'digitization' step which simulates only the noise but not the electronic signal reconstruction in the detector. Other applications could be mentioned such as educational applications. It should also emphasise that, although an inner detector is simulated, this simulation is really focussing on the calorimeter reconstruction (to make ckear that there is no real track reconstruction algorithms.}
\fdb{In addition to what Marumi said, I suggest to mention the fact that we trace the energy deposit in the calorimeter  so that one can develop supervised ML algorithms exploiting this feature. }

Algorithms incorporating machine learning (ML) are a new paradigm in reconstruction, calibration, identification and analysis of High Energy Physics (HEP) experimental data. In recent years, various ML architectures have been deployed to optimize low-level tasks such as clustering, reconstruction, fast simulation, pileup suppression and object identification. For example, ML-based fast calorimeter simulation relies on accurate target data to train a fast surrogate model of the forward process $T\rightarrow D$, where $T$ denotes the true set of stable final state particles produced in the collision and $D$ is the set of resulting detector hits. In particle reconstruction, on the other hand, the inverse process $D \rightarrow T$ is modelled by predicting a set of particles $R(D)$ to recover $T$ as accurately as possible. The development of such algorithms requires a realistic simulation of particle detector response $D(T)$ going beyond the parameterized momentum smearing used in studies of particle physics phenomenology~\cite{Mertens:2015kba}. 
In particular due to the complexity of particle showers in calorimeters, a detailed, microscopic simulation of interactions between particles and detector material is needed in order to develop low-level ML algorithms exploiting such features.

\sg{Recent research efforts to study calorimeter shower properties using ML~\cite{PhysRevD.97.014021,Qasim_2019,Di_Bello_2021} made use of \textsc{Geant4}-based simulation using simplified detector geometry. However an open source simulation with a realistic cylinder like hermetic geometry and realistic detector is yet to be adapted by HEP community for ML studies and beyond.}
% Accordingly, recent research efforts to distinguish shower profiles caused by different particles in dense material~\cite{PhysRevD.97.014021,Qasim_2019,Di_Bello_2021} made use of \textsc{Geant4}-based simulation. However, such studies have largely been limited to simplified detector scenarios such as rectangular blocks with uniform segmentation (for example in \cite{Di_Bello_2021}).
% Actual detectors, for example at the LHC, are significantly more complex, typically comprising multiple in-homogeneous layers of active, passive, and support materials arranged in a nearly hermetic cylindrical geometry. 
%There relevant for the performance of particle reconstruction
%and simulation algorithms in view of the needs of large experimental collaborations,
%e.g. at the LHC.
In an effort to close this gap, this letter presents the CalOrimeter Simulation for Ai applications (\scd{}), which uses \textsc{Geant4} to implement full shower simulation for particles in a full-coverage, highly-segmented sensitive volume comparable to that of multipurpose detectors at the LHC. \sg{The emphasis of this software package is on realistic calorimeter simulation. No realistic digitization and electronic readouts are implemented and energy loss due to these processes are neglected in this package.}
The program source code is linked together with a technical documentation on the project website\footnote{\url{https://scd-hep.readthedocs.io/en/latest/index.html}}.
\textsc{Geant4} simulation toolkit~\cite{ALLISON2016186} to simulate these interactions with high precision. \mk{This paragraph should be removed as there has been much much more than this in calorimeter simulation in the litterature.}
$\Rightarrow$ \sg{Addressed.}

The major components of the \scd{} are its electromagnetic (ECAL) and hadronic calorimeter (HCAL), designed to suit the needs of hadron collision analysis.
Single particle responses of the \scd{} calorimeters closely match those of the multipurpose LHC detectors. 
The main parameters of the calorimeters are largely configurable, including their material, granularity, depth and the amount of readout noise.
%This noise is added randomly to the calorimeter cell energies, approximating effects of digital readout.
The \scd{} also includes an inner tracking system (ITS) made of silicon tracking and supporting iron layers, the incorporation of which is subject to the choice of the user as well.
The ITS merely serves the purpose of simulating particle energy depositions upstream of the calorimeter, rather than a detailed tracking by means of individual detector hits.
The region between the beam axis and calorimeter system is filled with a magnetic field of adjustable strength.
Output data from the \scd{} are conveniently interfaced to standard topological clustering and jet clustering algorithms.
In consequence, the \scd{} allows to create datasets for the development of new particle reconstruction and simulation algorithms and has already been deployed in two such applications \cite{DiBello:2022rss,DiBello:2022iwf}.
%\textbf{[TODO: include PFlow and FastSim paper citations. \sg{$\rightarrow$ done.}]}

\mk{the introduction is where the notations in the same form as the other articles should be introduced, the other papers will then connect naturally with this one and the data will be expressed in a language that is easily understandable by ML community (that is a goal of this paper).}

\sg{$\Rightarrow$ the symbols in introduction is compatible with fastsim draft.}

% \mk{You can also state in the introduction that event displays are also part of the tool.} ==> Done

The default geometry is also provided in a format to be loaded in the Phoenix event display software, along with a script for exporting event output files for visualization.
